A Nearly Optimal Size Coreset Algorithm with Nearly Linear Time

A coreset is a point set containing information about geometric properties of a larger point set. A series of previous works show that in many machine learning problems, especially in clustering problems, coreset could be very useful to build efficient algorithms. Two main measures of an coreset construction algorithm's performance are the running time of the algorithm and the size of the coreset output by the algorithm. In this paper we study the construction of coresets for the $(k,z)$-clustering problem, which is a generalization of $k$-means and $k$-median problem. By properly designing a sketching-based distance estimation data structure, we propose faster algorithms that construct coresets with matching size of the state-of-the-art results.

==> settings.tex <==
\usepackage{amsmath,amsthm,amssymb}
\usepackage{fullpage}
\usepackage{mathtools,bbm,xspace}
\usepackage{mathrsfs}
\usepackage{bm}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage[dvipsnames]{xcolor}
\usepackage{subfig}
\usepackage{ifxetex}

\usepackage{verbatim}
\usepackage[
letterpaper,
top=1in,
bottom=1in,
left=1in,
right=1in]{geometry}

\ifxetex
\usepackage[bigdelims,vvarbb]{newpxmath}
\usepackage{mathspec}
\setallmainfonts(Digits,Latin){Noto Serif}
\else
\usepackage{mathpazo}
\fi

\usepackage[pagebackref]{hyperref}
\hypersetup{
pagebackref,
letterpaper=true,
colorlinks=true,
urlcolor=blue,
linkcolor=blue,
citecolor=OliveGreen,
}
\linespread{1.08}

\usepackage[capitalise,nameinlink]{cleveref}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{fact}{Fact}{Facts}
\crefname{theorem}{Theorem}{Theorems}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{claim}{Claim}{Claims}
\crefname{example}{Example}{Examples}
\crefname{problem}{Problem}{Problems}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{subsection}{Subsection}{Subsections}
\crefname{section}{Section}{Sections}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{itheorem}{Theorem}

\newtheorem{subclaim}{Claim}[theorem]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{openquestion}[theorem]{Open Question}
% \newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{protocol}[theorem]{Protocol}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{exercise-easy}[theorem]{Exercise}
\newtheorem{exercise-med}[theorem]{Exercise}
\newtheorem{exercise-hard}[theorem]{Exercise$^\star$}
\newtheorem{claim}[theorem]{Claim}

\newtheorem{remark}[theorem]{Remark}
\newtheorem{observation}[theorem]{Observation}

\allowdisplaybreaks

% Norm Stuff
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator*{\Tr}{\bm{Tr}}
\DeclareMathOperator*{\sgn}{sgn}

\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}

\newcommand{\svd}{\mathsf{SVDE}}
\newcommand{\onenorm}[1]{\norm{#1}_1}
\newcommand{\twonorm}[1]{\norm{#1}_2}
\newcommand{\infnorm}[1]{\norm{#1}_\infty}
\newcommand{\trnorm}[1]{\norm{#1}_{\ast}}

\DeclarePairedDelimiterX{\abs}[1]{\lvert}{\rvert}{#1}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\DeclareMathOperator*{\sign}{sign}

\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\mrm}[1]{\mathrm{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\C}{\mathbb{C}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}

\newcommand{\sym}[1][n]{\mathbb{S}^{#1}}
\newcommand{\psd}[1][n]{\mathbb{S}_+^{#1}}
\newcommand{\lprp}[1]{\left(#1\right)}
\newcommand{\lbrb}[1]{\left\{#1\right\}}
\newcommand{\lsrs}[1]{\left[#1\right]}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}

\newcommand{\eps}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\Ot}{\widetilde{O}}

\newcommand{\median}{\mathrm{Median}}
\newcommand{\diam}{\mathrm{Diam}}
\newcommand{\unif}{\mathrm{Unif}}
\newcommand{\supp}{\mathrm{Supp}}

\DeclareMathOperator*{\vol}{Vol}

% changing the following can be used to toggle author notes between on and off
\def\authornotes{1pt}

\ifdim\authornotes=1pt
\newcommand{\ynote}[1]{\footnote{\color{ForestGreen}Yeshwanth: #1}}
\newcommand{\jnote}[1]{\footnote{\color{Orange}Jelani: #1}}
\else
\newcommand{\ynote}[1]{}
\newcommand{\jnote}[1]{}
\fi

\usepackage{tikz}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% Paper Specific Commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\prodKernEmbedDS}{Produce Kernel Embedding Data Structure}
\newcommand{\prodKernEmbed}{Produce Kernel Embedding}
\newcommand{\kernEmbedRep}{\widetilde{\Omega} \left( \eps^{-2} \diam (\mathcal{W})^2 \log 1 / \delta \right)}

\newcommand{\cdfEmbedRep}{C \eps^{-4} \log^5 (d / \eps) \log 1 / \delta}
\newcommand{\cdfSlope}{\frac{128}{\eps}}
\newcommand{\cdfRes}{\left(\frac{\eps}{10d}\right)^3}
\newcommand{\cdfWid}{\left(10 \sqrt{\log (d / \eps)}\right)^3}
\newcommand{\cdfSens}{\left(\frac{\eps}{10d}\right)^3}
\newcommand{\cdfAcc}{\left(\frac{\eps}{256 \log (d / \eps)}\right)}
\newcommand{\cdfNSplits}{32 \log (d / \eps)}

\newcommand{\lipEmbedRep}{C \eps^{-2} \log^5 (d / \eps) \log 1 / \delta}
\newcommand{\lipSlope}{\frac{128}{\eps}}
\newcommand{\lipRes}{\left(\frac{\eps}{10d}\right)^3}
\newcommand{\lipWid}{\left(10 \sqrt{\log (d / \eps)}\right)^6}
\newcommand{\lipWidLoss}{\left(10 \sqrt{\log (d / \eps)}\right)^3}
\newcommand{\lipSens}{\left(\frac{\eps}{10d}\right)^3}
\newcommand{\lipAcc}{\left(\frac{\eps}{256 \log (d / \eps)}\right)}
\newcommand{\lipNSplits}{32 \log (d / \eps)}

\newcommand{\prodDEDS}{Produce Distance Estimation Data Structure}
\newcommand{\prodDE}{Produce Distance Estimates}
\newcommand{\updateDE}{Update Distance Estimation Data Structure}
\newcommand{\distEstRep}{\wt{\Omega} (\eps^{-2} \log 1 / \delta)}
\newcommand{\distEstSamps}{\wt{\Omega} (\eps^{-2} \log 1 / \delta)}
% \newcommand{\distEstQuant}{1 / \poly \left(\log (d / \eps)\right)}

\DeclareMathOperator{\quant}{Quant}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Diag}{Diag}

\newcommand{\queryProcP}{Process Query}

==> sym_norm.tex <==
\begin{theorem}[Symmetric norm version of Theorem~\ref{thm:subspace}]
	\label{thm:subspace_sym_norm}
	Given a dataset $X$ of $n$ points in $\R^d$, $\eps,\delta \in (0,0.5)$, and integer $k \geq 1$, suppose $\sigma: X \rightarrow \R_{\geq 0}$ is a sensitivity function satisfying thats
	\begin{align*}
	    \sigma(x) \geq \sup_{P\subseteq \mathcal{P}} \frac{d_{\ell}(x, P)}{\sum_{y\in X} d_{\ell}(y, P)}
	\end{align*}
	for each $x\in X$. Let $\G = \sum_{x\in X} \sigma(x)$ denote the total sensitivity. Suppose $S\subseteq X$ is constructed by taking 
	\begin{align*}
	    O( \eps^{-2} \G^2 \cdot (\eps^{-1} k^3\log (k/\eps)+\log(1/\delta)))
	\end{align*}
	samples, where each sample $x\in X$ is selected with probability $\frac{\sigma(x)}{\G}$ and has weight $w(x):= \frac{\G}{|S|\cdot \sigma(x)}$.
	%
	Then with probability at least $1-\delta$, $S$ is an $\eps$-weak-coreset for the $(k,z)$-subspace approximation problem over $X$.
	%
\end{theorem}



\begin{lemma}[Existence of approximate $k$-flats in low dimensional subspaces]
	\label{lem:projective_clustering}
	Given a weighted dataset $X$ of $n$ points together with weights $u(x)$ in $\R^d$, $ \eps \in (0,0.5)$, constant $z\geq 1$ and integer $k \geq 1$, there exists a $k$-flat $P$ that is spanned by at most $O(\eps^{-1} k^2 \log(k/\eps))$ points from $X$, such that 
	\begin{align*}
	    \sum_{x\in X} u(x)\cdot d_{\ell}(x,P)\leq (1+\eps)\cdot \min_{P'\in \mathcal{P}}\sum_{x\in X} u(x)\cdot d_{\ell}(x,P').
	\end{align*}
\end{lemma}
